ChipNet: Budget-Aware Pruning with Heaviside Continuous Approximations

Structured pruning methods are among the effective strategies for extracting small resource-efficient convolutional neural networks from their dense counterparts with minimal loss in accuracy. However, most existing methods still suffer from one or more limitations, that include 1) the need for training the dense model from scratch with pruning-related parameters embedded in the architecture, 2) requiring model-specific hyperparameter settings, 3) inability to include budget-related constraint in the training process, and 4) instability under scenarios of extreme pruning. In this paper, we present ChipNet, a deterministic pruning strategy that employs continuous Heaviside function and a novel crispness loss to identify a highly sparse network out of an existing dense network. Our choice of continuous Heaviside function is inspired by the field of design optimization, where the material distribution task is posed as a continuous optimization problem, but only discrete values (0 or 1) are practically feasible and expected as final outcomes. Our approach's flexible design facilitates its use with different choices of budget constraints while maintaining stability for very low target budgets. Experimental results show that ChipNet outperforms state-of-the-art structured pruning methods by remarkable margins of up to 16.1% in terms of accuracy. Further, we show that the masks obtained with ChipNet are transferable across datasets. For certain cases, it was observed that masks transferred from a model trained on feature-rich teacher dataset provide better performance on the student dataset than those obtained by directly pruning on the student data itself.

==> introduction.tex <==
\dpk{Arnav to add the remaining references in this section.} Convolution Neural Networks (CNNs) have resulted in several breakthroughs across various disciplines of  deep learning, especially for their effectiveness in extracting complex features which cannot be obtained using standard methods \citep{lecun1998gradient, Russakovsky2015ImageNetLS, ronneberger2015u}. The general trend has been to design deeper and more complex models \citep{he2016deep, zagoruyko2016wide} to achieve state-of-the-art (SOTA) results on standard datasets like ImageNet and CIFAR100 \citep{Russakovsky2015ImageNetLS, Krizhevsky2009LearningML}. However, the resultant models demand significantly high computational budget, making it hard to use them on low-memory hardware platforms that require high-inference speed. An example is the ResNet-152 \citep{he2016deep} \rish{two times cited} architecture that uses 60 million parameters and more than 20 Giga float-point-operations (FLOPs) to infer on images of size $224 \times 224$ pixels.

Most of the existing deep networks are heavily over-parameterized resulting in high memory footprint \citep{frankle2018lottery} \rish{is it correct citation}. Several strategies have been proposed to tackle this challenge \rish{or issue?}, that include network pruning \cite{liu2018rethinking}, neural architecture search using methods such as reinforcement learning \citep{jaafra2019reinforcement}, vector quantization \citep{han2015deep}, among others. Among these, network pruning has proved to be very effective in designing small CNN architectures that perform at par with their dense counterparts. Network pruning refers to the process of removal of unimportant weights or filters from a network and training it further to obtain performance at par with the original dense counterpart \citep{Liu2017iccv}.\rish{Among these, network pruning has proved to be very effective in designing small CNN architectures that perform at par with their dense counterparts.} %%Redundent hogya na thoda??

CNNs constitute the major computational burden, and for these to benefit from high degree of parallelism, it is important the network has a regular structure. This is violated if neurons or the respective connection weights are removed in isolation. While such a strategy theoretically reduces the size of the model, computational requirements are still the same \citep{Lemaire2019cvpr}. For effectively reducing the memory footprints, \emph{structured pruning} methods are better suited. These generally involve identifying less important feature maps using a predefined criterion and dropping them in the pruning stage, followed by further training of the sparse network.

\AC{Below paragraphs is somewhat redundant with related works section}
Several structured pruning approaches have been proposed in the recent literature. Among these, methods that learn the sparsity as a part of training have been more effective \citep{louizos2017learning, wen2016learning, pan2016dropneuron, alvarez2016learning, alvarez2017compression}. Further, a general consensus is that variational approaches perform better than others \citep{zhao2019variational, Lemaire2019cvpr}. One drawback with some of the existing methods is that they cannot be directly used on pretrained dense networks, and the additional pruning-related variables need to be embedded into the network in the early training process \cite{X}. Others require choosing hyperparamters based on the choice of the network, and are hard to adapt to new models \cite{X}. Further, with most of these, controlled pruning cannot be performed, and a resource-usage constraint can only be satisfied through trial-and-error approach. This requires training the network multiple times with different hyperparameters \cite{}. 

\dpk{Needs work here based on discussion: Me.}Recently, \citet{Lemaire2019cvpr} presented a budget-aware pruning method that includes the budget constraint as a part of the training process. However, this method is restricted to the choice of the budget constraint. Also, this approach as well as other recent methods are unstable for high sparsity cases, and require additional tricks to work. Overall, a general budget-aware pruning approach that can be coupled with different budget constraints as well as which is applicable to various networks with minimal modifications, is still missing in the existing literature.

% \dpk{Several pruning ways exist and ...Variational approaches perform better over deterministic schemes. Recent such approach also allows imposing a volume-budget constraint} Text here \dpk{Some drawbacks of the existing: 1) Most existing methods cannot be directly applied on the existing dense pretrained networks, and generally require retraining the larger network with a added variables. 2) Very model-specific and require choosing hyperparameters based on the choice of the architecture, 3) Methods such as BAR that include budget constraint are very restrictive to the choice of the budget, and may not necessarily provide an effectively optimized level of sparsity. 4) Depends on additional inputs such as knowledge distillation, 5) not very stable at high levels of sparsity and require additional hard-coding to stabilize.}

In this paper, we present ChipNet, a deterministic strategy for structured pruning that employs continuous Heaviside functions and crispness loss to identify a highly sparse network out of an existing pretrained dense network. The abbreviation `ChipNet' stands for Continuous Heaviside Pruning of Networks. Our pruning strategy draws inspiration from the field of design optimization, where the material distribution task is posed as a continuous optimization problem, but only discrete values \mbox{(0 or 1)} are practically feasible. Thus, only such values are produced as final outcomes through continuous Heaviside projections. We use a similar strategy to obtain the masks in our sparsity learning approach. The flexible design of ChipNet facilitates its use with different choices of budget constraints, such as restriction on the maximum number of parameters, or feature-channels or the volume of activations in the network. Through experiments on two popular architectures, we show that ChipNet consistently outperforms state-of-the-art pruning methods for different choices of budget constraints. 

ChipNet is very stable for even very low resource budgets, and we demonstrate this through experiments where network is pruned to as low as 1\% of the parameters from the original network. We show that for such extreme cases, ChipNet outperforms the respective baselines by remarkable margins, with an difference in accuracy of slightly beyond 16\% observed for one of the experiments. The masks learnt by ChipNet are transferable across datasets. We show that for certain cases, masks transferred from a model trained on feature-rich teacher dataset provide better performance on the student dataset than those obtained by directly pruning on the student data itself.



==> workflow.tex <==


\begin{algorithm}[H]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}

\Input{pretrained network weights $\mathbf{W}$; \Comment{Get weights of the pretrained network} \\
budget constraint function $\mathcal{V}(\mathbf{\cdot})$; budget value $\mathcal{V}_0$; budget constrain $\mathcal{B}$;\\
training data $\mathcal{D}$; pruning iterations $N$} 
\Output{learnt sparsity masks $\mathbf{z}_h$}
$\psi_i \in \Psi \leftarrow$ random initialization \\
\For {$k = 1 \hdots N$} 
{
    \State $(x, y) \gets \mathcal{D}$
    \State $\tilde{z} \gets Logistic(\psi)$
    \State $z \gets ContinuousHeaviside(\tilde{z})$
    \State $\bar{y} \gets Forward(x, \mathbf{W}, z)$
    \State $\mathcal{V}^{(\mathcal{B})} \gets \mathcal{V}(z, \mathcal{B})$
    \State $\mathcal{L} \gets ChipNetLoss(\mathcal{V}^{(\mathcal{B})}, \mathcal{V}_0, \tilde{z}, z, \Bar{y}, y)$
    \State $(\nabla{\mathbf{W}}, \nabla{\psi}) \gets Backward(\mathcal{L})$
    \State $(\mathbf{W}, \psi)\gets OptimizationStep(\nabla{\mathbf{W}}, \nabla{\psi})$
    
%${}^{k}x_{i}$ $\leftarrow$ NORMALIZE(${}^{k}x_{i}$)
 }
\caption{ChipNet Pruning Approach}
\end{algorithm}




